Controlled Text Reduction

Producing a reduced version of a source text, as in generic or focused summarization, inherently involves two distinct subtasks: deciding on targeted content and generating a coherent text conveying it. While some popular approaches address summarization as a single end-to-end task, prominent works support decomposed modeling for individual subtasks. Further, semi-automated text reduction is also very appealing, where users may identify targeted content while models would generate a corresponding coherent summary. In this paper, we focus on the second subtask, of generating coherent text given pre-selected content. Concretely, we formalize \textit{Controlled Text Reduction} as a standalone task, whose input is a source text with marked spans of targeted content ("highlighting"). A model then needs to generate a coherent text that includes all and only the target information. We advocate the potential of such models, both for modular fully-automatic summarization, as well as for semi-automated human-in-the-loop use cases. Facilitating proper research, we crowdsource high-quality dev and test datasets for the task. Further, we automatically generate a larger "silver" training dataset from available summarization benchmarks, leveraging a pretrained summary-source alignment model. Finally, employing these datasets, we present a supervised baseline model, showing promising results and insightful analyses.

==> tables/agreement_results.tex <==
\begin{table}[]
\centering
\begin{tabular}{ccc}
\hline
IAA   & ARefA & IRefA \\ \hline
82.09 & 78.23 & 74.95 \\ \hline
\end{tabular}
\caption{Inter-Annotator-Agreement (IAA), annotator to reference agreement (ARefA), and Inter-Reference Agreement (IRefA) scores on all content tokens.}
\label{tab:agreement_scores}
\end{table}
